SpikeGS: Reconstruct 3D scene via fast-moving bio-inspired sensors

3D Gaussian Splatting (3DGS) demonstrates unparalleled superior performance in 3D scene reconstruction. However, 3DGS heavily relies on the sharp images. Fulfilling this requirement can be challenging in real-world scenarios especially when the camera moves fast, which severely limits the application of 3DGS. To address these challenges, we proposed Spike Gausian Splatting (SpikeGS), the first framework that integrates the spike streams into 3DGS pipeline to reconstruct 3D scenes via a fast-moving bio-inspired camera. With accumulation rasterization, interval supervision, and a specially designed pipeline, SpikeGS extracts detailed geometry and texture from high temporal resolution but texture lacking spike stream, reconstructs 3D scenes captured in 1 second. Extensive experiments on multiple synthetic and real-world datasets demonstrate the superiority of SpikeGS compared with existing spike-based and deblur 3D scene reconstruction methods. Codes and data will be released soon.

==> sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}

%
Reconstructing 3D scene from 2D images has long been a popular research topic. The emergence of Neural Radiance Fields \cite{nerf} (NeRF)  and 3D Gaussian Splatting \cite{3dgs} (3DGS) has propelled rapid advancements in this field. To ensure high-quality 3D reconstruction, users need to capture clear images of the scene (or object) from various poses. However, when mounted on high-speed vehicles, e.g., cars, drones, and trains, traditional cameras with low temporal resolution introduce significant motion blur, which severely limits the method's ability to accurately understand 3D scenes.
%为了确保高质量的3d重建，用户需要在不同的角度对场景(or 物体)拍摄清晰的图像。然而，在高速场景中, 例如自动驾驶，有着低时间分辨率的传统相机会引入严重的运动模糊那大大限制了significantly limit the quality of novel view synthesis (NVS).  
%然而，在高速载具上时，traditional cameras with low temporal resolution introduce significant motion blur
%


%To address this issue, some work [] start to explore the use of neuromorphic cameras for 3D reconstruction and have made notable progress [].

Recently, neuromorphic cameras with high-temporal resolution, e.g., event cameras \cite{dvs1, dvs2, dvs3, dvs4, dvs5} and spike cameras \cite{spikecamera, spikecode}, have drawn significant attention in the 3D high-speed scenes reconstruction. Some studies \cite{rudnev2023eventnerf, hwang2023ev,wangevggs} attempt to obtain 3D scene representations directly from event streams. However, due to the differential sampling mechanism of event cameras,  event streams are hard to provide the texture information of objects. This constraint limits the effectiveness of these approaches. Hence, event streams often need to be combined with other modalities, such as images, to achieve high-quality 3D reconstruction \cite{xiong2024event3dgs, yu2024evagaussians}. Different from event cameras, spike cameras can accumulate light intensity and output binary spike streams to record texture details. Consequently, spike cameras have demonstrated superiority in various high-speed computer vision tasks without adding other modality data \cite{2022scflow,2022spkTransformer,Spk2ImgNet}. %后面一定补充引用！！！！

%最近，有着高时间分辨率的神经形态相机(including dvs and ivs)在3D \textbf{high-speed} scenes reconstruction中引起了广泛关注。一些工作尝试直接从事件相机的事件流中获得3D scene representation. 然而，事件相机由于其差分采样的机制本身难以捕捉物体的纹理信息[]. 这constrained the effectiveness of these approaches, resulting in limited outcomes. 因此，事件流往往需要结合其他模态数据，例如图像，才能完成高质量的3d高速场景重建[]。 不同于事件相机, Spike camera 能累积光强and output binary spike streams to \textbf{record object textures detilas}. Consequently, 脉冲相机 can be applied in various high-speed computer vision task without 其他模态数据.  
Sensing the potential of spike cameras for 3D  high-speed scene reconstruction, Spike-NeRF\cite{guo2024spike} and SpikeNeRF\cite{zhu2024spikenerf} are first proposed. Although they have shown the feasibility of 3D scene reconstruction with spike cameras, some challenges remain unresolved. For \cite{zhu2024spikenerf}, its main experiments are conducted in static scenes, making it challenging to demonstrate the effectiveness of SpikeNeRF on high-speed scenes. For \cite{guo2024spike}, it attempts to process high-speed dynamic scenes. However, its experiments are solely evaluated on synthetic datasets, making it challenging to demonstrate the generalization of Spike-NeRF on real scenes. Another challenge is that the above methods are computationally so inefficient, i.e., slow training speeds and an inability to render in real-time, due to the use of NeRF as a framework. 
%形容词

%另一个挑战是上述方法的计算效率非常高
%1.三维重建一直是一个热门的主题，许多优秀的工作通过使用nerf和gs取得了卓越的性能。然而受限于低帧率，在高速场景中传统相机捕获的模糊图像将大大限制重建的清晰度。为此，一些工作开始尝试使用神经形态相机进行三维重建and取得了一定进展。
%2.作为一种神经形态相机，脉冲相机具有高时间分辨率and能通过输出二进制脉冲流清晰地记录动态场景中的物体纹理。因此，它能广泛地被应用到各种高速场景的计算机视觉领域。窥探(嗅)到脉冲相机在高速场景中3d重建领域的潜力，[]首次提出了spike-nerf(=。spike nerf 的初衷是从运动的相机中获得3d场景表征。然而，它的实验被评估在静态的场景(场景和相机都是静止的)中，那是困难去证明xxx的。同期[]尝试从一段连续的脉冲流中重建3d场景。然而，它的实验仅仅被评估在合成数据集上 which 与真实脉冲流还存在一定的gap[].
%此外，上述两个方法都基于nerf，这导致他们的训练速度很慢，对开放场景效果不好，且不能实时渲染，严重限制了脉冲相机运用在3D重建的潜力。为此，
%尽管
%为什么要用3DGS(快速训练，实时渲染)

To address the mentioned challenges, we first combine \textbf{s}pike streams and 3D\textbf{GS} to design a tailored 3D reconstruction pipeline, \textbf{S}pike\textbf{GS}. With accumulation rasterization, interval supervision, and a specially designed pipeline, SpikeGS reconstructs detailed geometry and texture from high-temporal resolution but texture lacking spike stream as shown in Fig.~\ref{teasor}. 
Moreover, we provide novel 3D high-speed scene reconstruction datasets. Experiments on both real and synthetic data demonstrate the superiority of SpikeGS.
%在真实和合成数据上的实验都证明了x的优越性

%为了解决被提到的主要挑战，我们首次将脉冲流和3dgs结合起来，设计出了一个量体裁衣的3d重构pipline。具体地, 我们提出了一种快速且有效地脉冲流表征xxx，它能快速地估计光强信息并保留高速场景的时刻信息。进一步xxx将。

%Novel-view synthesis (NVS) is a long-standing problem aiming to render photo-realistic images from novel views of a scene from a sparse set of input images. This topic has recently seen impressive progress due to the use of neural networks to learnrepresentations that are well suited for view synthesis tasks, known as Neural Radiance Field (NeRF)\cite{nerf}. Despite its success, NeRF performs poorly in high-speed scenes since the motion blur caused by high-speed scenes violates the assumption by NeRF that the input images are in sharp focus. Deblur methods such as Deblur-NeRF \cite{ma2022deblur} can only handle mild motion blur. The introduction of high-speed neuromorphic cameras, such as event cameras \cite{liu2022devrf} and spike cameras, are expected to fundamentally solve this problem. 

%   \begin{figure}[htbp]
%     \centering
%     \includegraphics[width=\linewidth]{figures/f1_4.pdf}
%     \caption{ Existing works on NeRF (orange background) are reconstructed from image sequences generated by traditional cameras which record the luminance intensity during the exposure time at a fixed frame rate producing strong blur in high-speed scenes. Our approach (blue background) produces significantly better and sharper results by using dense spike streams instead of images sequences.}\label{f1_2}
% \end{figure}

The main contributions of this paper can be summarized as follows:
\begin{itemize}
\item[$\bullet$] SpikeGS, the first 3DGS approach designed for spike camera that enables a novel view synthesis for high-speed scenes.


\item[$\bullet$] Comprehensive datasets including both synthetic and real data with varying motion speeds.



\item[$\bullet$]  Empirically, we show the superiority of SpikeGS both on computational efficiency and reconstruction quality. 

\end{itemize}


==> sec/1_intro_2.tex <==
\section{Introduction}
\label{sec:intro}

%
Reconstructing 3D scene from 2D images has long been a popular research topic. The emergence of Neural Radiance Fields \cite{nerf} (NeRF)  and 3D Gaussian Splatting \cite{3dgs} (3DGS) has propelled rapid advancements in this field. To ensure high-quality 3D reconstruction, users need to capture clear images of the scene (or object) from various poses. However, when mounted on high-speed vehicles, e.g., cars, drones, and trains, traditional cameras with low temporal resolution introduce significant motion blur, which severely limits the method's ability to accurately understand 3D scenes.
%为了确保高质量的3d重建，用户需要在不同的角度对场景(or 物体)拍摄清晰的图像。然而，在高速场景中, 例如自动驾驶，有着低时间分辨率的传统相机会引入严重的运动模糊那大大限制了significantly limit the quality of novel view synthesis (NVS).  
%然而，在高速载具上时，traditional cameras with low temporal resolution introduce significant motion blur
%


%To address this issue, some work [] start to explore the use of neuromorphic cameras for 3D reconstruction and have made notable progress [].

Recently, neuromorphic cameras with high-temporal resolution, e.g., event cameras \cite{dvs1, dvs2, dvs3, dvs4, dvs5} and spike cameras \cite{spikecamera, spikecode}, have drawn significant attention in the 3D high-speed scenes reconstruction. Some studies \cite{rudnev2023eventnerf, hwang2023ev,wangevggs} attempt to obtain 3D scene representations directly from event streams. However, due to the differential sampling mechanism of event cameras,  event streams are hard to provide the texture information of objects. This constraint limits the effectiveness of these approaches. Hence, event streams often need to be combined with other modalities, such as images, to achieve high-quality 3D reconstruction \cite{xiong2024event3dgs, yu2024evagaussians}.  %后面一定补充引用！！！！

%最近，有着高时间分辨率的神经形态相机(including dvs and ivs)在3D \textbf{high-speed} scenes reconstruction中引起了广泛关注。一些工作尝试直接从事件相机的事件流中获得3D scene representation. 然而，事件相机由于其差分采样的机制本身难以捕捉物体的纹理信息[]. 这constrained the effectiveness of these approaches, resulting in limited outcomes. 因此，事件流往往需要结合其他模态数据，例如图像，才能完成高质量的3d高速场景重建[]。 不同于事件相机, Spike camera 能累积光强and output binary spike streams to \textbf{record object textures detilas}. Consequently, 脉冲相机 can be applied in various high-speed computer vision task without 其他模态数据.  
Different from event cameras, spike cameras can accumulate light intensity and output binary spike streams to record texture details. Sensing the potential of spike cameras for 3D  high-speed scene reconstruction, Spike-NeRF\cite{guo2024spike} and SpikeNeRF\cite{zhu2024spikenerf} are first proposed. Although they have shown the feasibility of 3D scene reconstruction with spike cameras, some challenges remain unresolved. For \cite{zhu2024spikenerf}, its main experiments are conducted in static scenes with Gray-scale, making it challenging to demonstrate the effectiveness of SpikeNeRF on high-speed RGB scenes. For \cite{guo2024spike}, it attempts to process high-speed dynamic scenes. However, its experiments are solely evaluated on synthetic datasets, making it challenging to demonstrate the generalization of Spike-NeRF on real scenes. Another challenge is that the above methods are computationally so inefficient, i.e., slow training speeds and an inability to render in real-time, due to the use of NeRF as a framework. 

%形容词

%另一个挑战是上述方法的计算效率非常高
%1.三维重建一直是一个热门的主题，许多优秀的工作通过使用nerf和gs取得了卓越的性能。然而受限于低帧率，在高速场景中传统相机捕获的模糊图像将大大限制重建的清晰度。为此，一些工作开始尝试使用神经形态相机进行三维重建and取得了一定进展。
%2.作为一种神经形态相机，脉冲相机具有高时间分辨率and能通过输出二进制脉冲流清晰地记录动态场景中的物体纹理。因此，它能广泛地被应用到各种高速场景的计算机视觉领域。窥探(嗅)到脉冲相机在高速场景中3d重建领域的潜力，[]首次提出了spike-nerf(=。spike nerf 的初衷是从运动的相机中获得3d场景表征。然而，它的实验被评估在静态的场景(场景和相机都是静止的)中，那是困难去证明xxx的。同期[]尝试从一段连续的脉冲流中重建3d场景。然而，它的实验仅仅被评估在合成数据集上 which 与真实脉冲流还存在一定的gap[].
%此外，上述两个方法都基于nerf，这导致他们的训练速度很慢，对开放场景效果不好，且不能实时渲染，严重限制了脉冲相机运用在3D重建的潜力。为此，
%尽管
%为什么要用3DGS(快速训练，实时渲染)

To address the mentioned challenges, we first combine \textbf{s}pike streams and 3D\textbf{GS} to design a tailored 3D reconstruction pipeline, \textbf{S}pike\textbf{GS}. With accumulation rasterization, interval supervision, and a specially designed pipeline, SpikeGS reconstructs detailed geometry and texture from high-temporal resolution but texture lacking spike stream as shown in Fig.~\ref{teasor}. 
Moreover, we provide novel 3D high-speed scene reconstruction datasets. Experiments on both real and synthetic data demonstrate the superiority of SpikeGS.
%在真实和合成数据上的实验都证明了x的优越性

%为了解决被提到的主要挑战，我们首次将脉冲流和3dgs结合起来，设计出了一个量体裁衣的3d重构pipline。具体地, 我们提出了一种快速且有效地脉冲流表征xxx，它能快速地估计光强信息并保留高速场景的时刻信息。进一步xxx将。

%Novel-view synthesis (NVS) is a long-standing problem aiming to render photo-realistic images from novel views of a scene from a sparse set of input images. This topic has recently seen impressive progress due to the use of neural networks to learnrepresentations that are well suited for view synthesis tasks, known as Neural Radiance Field (NeRF)\cite{nerf}. Despite its success, NeRF performs poorly in high-speed scenes since the motion blur caused by high-speed scenes violates the assumption by NeRF that the input images are in sharp focus. Deblur methods such as Deblur-NeRF \cite{ma2022deblur} can only handle mild motion blur. The introduction of high-speed neuromorphic cameras, such as event cameras \cite{liu2022devrf} and spike cameras, are expected to fundamentally solve this problem. 

%   \begin{figure}[htbp]
%     \centering
%     \includegraphics[width=\linewidth]{figures/f1_4.pdf}
%     \caption{ Existing works on NeRF (orange background) are reconstructed from image sequences generated by traditional cameras which record the luminance intensity during the exposure time at a fixed frame rate producing strong blur in high-speed scenes. Our approach (blue background) produces significantly better and sharper results by using dense spike streams instead of images sequences.}\label{f1_2}
% \end{figure}

The main contributions of this paper can be summarized as follows:
\begin{itemize}
\item[$\bullet$] SpikeGS, the first framework that integrates the spike
streams into 3DGS pipeline to reconstruct 3D scenes via a fast-
moving bio-inspired camera. Our method is designed for spike-based-only supervision which is highly robust
to various speeds.


\item[$\bullet$] The first datasets include both synthetic and real RGB spike data with varying motion speeds. We will publicly release our code and dataset for future research.



\item[$\bullet$]  Empirically, we show the superiority of SpikeGS both on computational efficiency and reconstruction quality. 

\end{itemize}
% 速度是3D重建领域最受关注的问题之一。NeRF虽然极大的推动了3D重建的发展，但是其令人难以忍受的训练和渲染速度一直饱受诟病。3DGS完美的解决了这一问题,将重建速度改善至分钟级并且实现了实时渲染，instantsolat更是将重建速度提升至秒级。但是，极快的重建速度并不意味着实现实时的重建。3DGS和大多数基于3DGS的方法需要锐利的图像输入，这意味着捕获一个最简单的场景也需要30s甚至更长的时间————因为相机只能缓慢运动以防止运动模糊。在不远的将来，限制3D重建速度的将不再是训练速度，而是相机捕获场景的速度。即使当下，对锐利图像的需求也限制3DGS应用在重建无人机或者快速运动的汽车捕获的场景上。
% 许多deblur的方法尝试解决上述问题，然而受限于传统相机的感光特性，能处理的motion blur非常有限。Bio-inspired came因其超高的时间分辨率被认为有望彻底解决上述问题。作为Bio-inspired cmera的代表，事件流相机和脉冲相机已经被广泛的运用于高速场景的3D重建，并且取得了显著的成效。然而，由于事件流本身纹理极度匮乏，基于事件流相机的方法往往需要联合RGB相机进行重建，严重限制了其应用。Spike Camera能捕捉丰富的视觉纹理，被认为更适合独立进行3D重建。然而之前的方案无法重建真实的彩色数据，也从未在实拍的高速场景下进行过测试，其训练和渲染效率更是远低于基于3DGS的方法，实用性有待商榷。
% 在本文中，我们combine spike streams and 3DGS to design a tailored 3D reconstruction pipeline,首次实现了重建脉冲相机在一秒内捕获的场景。With accumulation rasterization, interval supervision, and a specially designed pipeline, SpikeGS reconstructs detailed geometry and texture from high-temporal resolution but texture lacking spike stream as shown in Fig.1. 为了验证我们的方案，我们拍摄了第一个用于3D重建的高速运动的脉冲数据集，这也是第一个用于3D重建的彩色脉冲数据集。实验表明，我们的方法的3D重建效果不仅在高速场景中由于目前所有的方法，对速度的鲁棒性也非常优异。我们的主要贡献如下： 
% SpikeGS, the first framework that integrates the spike
% streams into 3DGS pipeline to reconstruct 3D scenes via a fast-
% moving bio-inspired camera. Our method is designed for spike-based-only supervision which is highly robust
% to various speeds.
% SpikeGS-dataset, 第一个用于3D重建的高速脉冲数据集，第一个用于3D重建的彩色脉冲数据集，第一个有明确速度标注和同一场景不同速度的脉冲数据集。我们还提供了一个拍摄室内高速脉冲3D重建场景的标准范式
% 实验表明，我们的方法的3D重建效果不仅在高速场景中由于目前所有的方法，对速度的鲁棒性也非常优异。我们在仿真数据集上首次验证了脉冲相机重建开放户外场景的可能性。

==> sec/checklist.tex <==
\section{checklist}
\label{sec:checklist}
Unless specified otherwise, please answer “yes” to each question if the relevant information is described either in the paper itself or in a technical appendix with an explicit reference from the main paper. If you wish to explain an answer further, please do so in a section titled “Reproducibility Checklist” at the end of the technical appendix.

This paper
\begin{itemize}
\item[$\bullet$]Includes a conceptual outline and/or pseudocode description of AI methods introduced (yes)

\item[$\bullet$]Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results (yes)

\item[$\bullet$]Provides well marked pedagogical references for less-familiare readers to gain background necessary to replicate the paper (yes)

\item[$\bullet$]Does this paper make theoretical contributions? (yes)
\end{itemize}

If yes, please complete the list below.
\begin{itemize}
\item[$\bullet$]All assumptions and restrictions are stated clearly and formally. (yes)

\item[$\bullet$]All novel claims are stated formally (e.g., in theorem statements). (yes)

\item[$\bullet$]Proofs of all novel claims are included. (yes)

\item[$\bullet$]Proof sketches or intuitions are given for complex and/or novel results. (yes)

\item[$\bullet$]Appropriate citations to theoretical tools used are given. (yes)

\item[$\bullet$]All theoretical claims are demonstrated empirically to hold. (yes)

\item[$\bullet$]All experimental code used to eliminate or disprove claims is included. (yes)

\item[$\bullet$]Does this paper rely on one or more datasets? (yes)
\end{itemize}

 
If yes, please complete the list below.
\begin{itemize}
 
\item[$\bullet$]A motivation is given for why the experiments are conducted on the selected datasets (yes)

\item[$\bullet$]All novel datasets introduced in this paper are included in a data appendix. (yes)

\item[$\bullet$]All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (yes)

\item[$\bullet$]All datasets drawn from the existing literature (potentially including authors’ own previously published work) are accompanied by appropriate citations. (yes)
\item[$\bullet$]All datasets drawn from the existing literature (potentially including authors’ own previously published work) are publicly available. (yes)
\item[$\bullet$]All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisficing. (yes)
\item[$\bullet$]Does this paper include computational experiments? (yes)
\end{itemize}
If yes, please complete the list below.
\begin{itemize}
\item[$\bullet$]Any code required for pre-processing data is included in the appendix. (yes).
\item[$\bullet$]All source code required for conducting and analyzing the experiments is included in a code appendix. (yes)
\item[$\bullet$]All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (yes)
\item[$\bullet$]All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from (yes)
\item[$\bullet$]If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results. (yes)
\item[$\bullet$]This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks. (yes)
\item[$\bullet$]This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics. (yes)
\item[$\bullet$]This paper states the number of algorithm runs used to compute each reported result. (yes)
\item[$\bullet$]Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information. (yes)
\item[$\bullet$]The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank). (yes)
\item[$\bullet$]This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments. (yes)
\item[$\bullet$]This paper states the number and range of values tried per (hyper-) parameter during development of the paper, along with the criterion used for selecting the final parameter setting. (NA)
\end{itemize}
